First Order Decision Diagrams for Relational MDPs

Markov decision processes capture sequential decision making under uncertainty, where an agent must choose actions so as to optimize long term reward. The paper studies efficient reasoning mechanisms for Relational Markov Decision Processes (RMDP) where world states have an internal relational structure that can be naturally described in terms of objects and relations among them. Two contributions are presented. First, the paper develops First Order Decision Diagrams (FODD), a new compact representation for functions over relational structures, together with a set of operators to combine FODDs, and novel reduction techniques to keep the representation small. Second, the paper shows how FODDs can be used to develop solutions for RMDPs, where reasoning is performed at the abstract level and the resulting optimal policy is independent of domain size (number of objects) or instantiation. In particular, a variant of the value iteration algorithm is developed by using special operations over FODDs, and the algorithm is shown to converge to the optimal policy.

==> temp <==
This is TeX, Version 3.14159 (Web2C 7.3.1)
(wang08a.tex
LaTeX2e <2000/06/01>
Babel <v3.7h> and hyphenation patterns for american, french, german, ngerman, i
talian, nohyphenation, loaded.
(/usr/share/texmf/tex/latex/base/latex209.def

          Entering LaTeX 2.09 COMPATIBILITY MODE
 *************************************************************
    !!WARNING!!    !!WARNING!!    !!WARNING!!    !!WARNING!!   
 
 This mode attempts to provide an emulation of the LaTeX 2.09
 author environment so that OLD documents can be successfully
 processed. It should NOT be used for NEW documents!
 
 New documents should use Standard LaTeX conventions and start
 with the \documentclass command.
 
 Compatibility mode is UNLIKELY TO WORK with LaTeX 2.09 style
 files that change any internal macros, especially not with
 those that change the FONT SELECTION or OUTPUT ROUTINES.
 
 Therefore such style files MUST BE UPDATED to use
          Current Standard LaTeX: LaTeX2e.
 If you suspect that you may be using such a style file, which
 is probably very, very old by now, then you should attempt to
 get it updated by sending a copy of this error message to the
 author of that file.
 *************************************************************

(/usr/share/texmf/tex/latex/base/tracefnt.sty)
(/usr/share/texmf/tex/latex/base/latexsym.sty)
(/usr/share/texmf/tex/latex/config/latex209.cfg)
(/usr/share/texmf/tex/latex/tools/rawfonts.sty
(/usr/share/texmf/tex/latex/tools/somedefs.sty)
(/usr/share/texmf/tex/latex/base/ulasy.fd)))
(/usr/share/texmf/tex/latex/base/article.cls
Document Class: article 2000/05/19 v1.4b Standard LaTeX document class
(/usr/share/texmf/tex/latex/base/size11.clo)) (jair.sty
Document Style `jair' -- May 1993.
) (theapa.sty) (/usr/share/texmf/tex/plain/dvips/epsf.tex
This is `epsf.tex' v2.7k <10 July 1997>
) (/usr/share/texmf/tex/generic/misc/psfig.sty
psfig/tex 1.10-dvips
) (wang08a.aux)
Underfull \vbox (badness 1237) has occurred while \output is active
(/usr/share/texmf/tex/latex/base/omscmr.fd) [1] [2]
Overfull \hbox (2.96509pt too wide) in paragraph at lines 240--253
\OT1/cmr/m/n/10.95 ing, Ot-terlo, & Raedt, 2004), and first or-der value it-er-
a-tion (FOVIA) (Gro^^Y-mann, H^^?olldobler,
[3] [4] [5]
psfig: searching Regressunload.eps for bounding box
psfig: including Regressunload.eps 
[6] [7]
psfig: searching semantics.eps for bounding box
psfig: including semantics.eps 
[8] [9] [10] [11]
psfig: searching reduced.eps for bounding box
psfig: including reduced.eps 
psfig: searching combineFODD.eps for bounding box
psfig: including combineFODD.eps 
[12] [13] [14] [15]
psfig: searching R7replacew0.eps for bounding box
psfig: including R7replacew0.eps 
psfig: searching R7remove.eps for bounding box
psfig: including R7remove.eps 
[16] [17] [18]
psfig: searching R7order.eps for bounding box
psfig: including R7order.eps 
[19]
psfig: searching R7order3.eps for bounding box
psfig: including R7order3.eps 
psfig: searching minsetvar.eps for bounding box
psfig: including minsetvar.eps 

Underfull \vbox (badness 10000) has occurred while \output is active [20]
psfig: searching unification.eps for bounding box
psfig: including unification.eps 
[21]
psfig: searching eqRed1.eps for bounding box
psfig: including eqRed1.eps 
[22] [23]
Overfull \hbox (11.81825pt too wide) in paragraph at lines 1796--1799
[]\OT1/cmr/m/n/10.95 Finally, by the def-i-ni-tion of $[]$, $[][] [][](\OML/cmm
/m/it/10.95 I; ^^P\OT1/cmr/m/n/10.95 ) = [][] [][] [][](\OML/cmm/m/it/10.95 I; 
^^P\OT1/cmr/m/n/10.95 ) =
[24]
psfig: searching tvdtemplate.eps for bounding box
psfig: including tvdtemplate.eps 
psfig: searching logisticstvds.eps for bounding box
psfig: including logisticstvds.eps 

Underfull \hbox (badness 2065) in paragraph at lines 1953--1953
[]\OT1/cmr/m/n/10.95 FODDs for lo-gis-tics do-main: TVDs, ac-tion choice, and r
e-ward func-
[25] [26]
psfig: searching bigprob.eps for bounding box
psfig: including bigprob.eps 
[27] [28] [29]
psfig: searching novarinTVD.eps for bounding box
psfig: including novarinTVD.eps 
[30]
psfig: searching stdapart.eps for bounding box
psfig: including stdapart.eps 
[31]
psfig: searching union.eps for bounding box
psfig: including union.eps 
[32]
Underfull \vbox (badness 2828) has occurred while \output is active [33]
psfig: searching labelOrdering.eps for bounding box
psfig: including labelOrdering.eps 
[34]
psfig: searching regression.eps for bounding box
psfig: including regression.eps 
[35]
Overfull \hbox (2.20703pt too wide) in paragraph at lines 2646--2658
\OT1/cmr/m/n/10.95 the re-sult of adding $[\OML/cmm/m/it/10.95 Pr\OT1/cmr/m/n/1
0.95 (\OML/cmm/m/it/10.95 unloadS\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 b[]; t
[]\OT1/cmr/m/n/10.95 )) \OMS/cmsy/m/n/10.95 
 \OML/cmm/m/it/10.95 Regr\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 V[]; unloadS\O
T1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 b[]; t[]\OT1/cmr/m/n/10.95 ))]$ to $[\OML
/cmm/m/it/10.95 Pr\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 unloadF\OT1/cmr/m/n/1
0.95 (\OML/cmm/m/it/10.95 b[]; t[]\OT1/cmr/m/n/10.95 ))$

Overfull \hbox (8.10023pt too wide) in paragraph at lines 2646--2658
\OMS/cmsy/m/n/10.95 
\OML/cmm/m/it/10.95 Regr\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 V[]; unloadF\OT
1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 b[]; t[]\OT1/cmr/m/n/10.95 ))]\OML/cmm/m/i
t/10.95 :$ \OT1/cmr/m/n/10.95 Note that we first stan-dard-ize apart di-a-grams
 for $\OML/cmm/m/it/10.95 unloadS\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 b[]; t
[]\OT1/cmr/m/n/10.95 )$

Overfull \hbox (4.89784pt too wide) in paragraph at lines 2694--2699
[]\OT1/cmr/bx/n/10.95 Figure 19[](i) \OT1/cmr/m/n/10.95 gives the re-duced re-s
ult of mul-ti-ply-ing Fig-ure 19[](h), $[](\OML/cmm/m/it/10.95 T[]\OT1/cmr/m/n/
10.95 )$,
[36] [37]
Overfull \hbox (0.89275pt too wide) in paragraph at lines 2718--2727
\OT1/cmr/m/n/10.95 the re-sult of block re-place-ment in re-gres-sion of $\OML/
cmm/m/it/10.95 V[]$ \OT1/cmr/m/n/10.95 through ac-tion al-ter-na-tive $\OML/cmm
/m/it/10.95 unloadS\OT1/cmr/m/n/10.95 (\OML/cmm/m/it/10.95 b[]; t[]\OT1/cmr/m/n
/10.95 )$.
[38]
psfig: searching copyop.eps for bounding box
psfig: including copyop.eps 
(wang08a.bbl [39] [40] [41]) [42] (wang08a.aux) )
(see the transcript file for additional information)
Output written on wang08a.dvi (42 pages, 177608 bytes).
Transcript written on wang08a.log.

